Instability and nonuniqueness for the $2d$ Euler equations in vorticity form, after M. Vishik

In this expository work, we present Vishik's theorem on non-unique weak solutions to the two-dimensional Euler equations on the whole space, \[ \partial_t \omega + u \cdot \nabla \omega = f \, , \quad u = \frac{1}{2\pi} \frac{x^\perp}{|x|^2} \ast \omega \, , \] with initial vorticity $\omega_0 \in L^1 \cap L^p$ and $f \in L^1_t (L^1 \cap L^p)_x$, $p < \infty$. His theorem demonstrates, in particular, the sharpness of the Yudovich class. An important intermediate step is the rigorous construction of an unstable vortex, which is of independent physical and mathematical interest. We follow the strategy of Vishik but allow ourselves certain deviations in the proof and substantial deviations in our presentation, which emphasizes the underlying dynamical point of view.

==> Figures/abstract.tex <==
% arXiv abstract, written by Dallas
% This isn't integrated into the main file.

% (Instability and non-uniqueness in the Cauchy problem for the Euler equations of an ideal incompressible fluid, 2018)

In this expository work, we present Vishik's theorem on non-unique weak solutions to the two-dimensional Euler equations on the whole space,
  \[ \partial_t \omega + u \cdot \nabla \omega = f \, , \quad u = \frac{1}{2\pi} \frac{x^\perp}{|x|^2} \ast \omega \, , \] with initial vorticity $\omega_0 \in L^1 \cap L^p$ and $f \in L^1_t (L^1 \cap L^p)_x$, $p < \infty$. His theorem demonstrates, in particular, the sharpness of the Yudovich class. An important intermediate step is the rigorous construction of an unstable vortex, which is of independent physical and mathematical interest. We follow the strategy of Vishik but allow ourselves certain deviations in the proof and substantial deviations in our presentation, which emphasizes the underlying dynamical point of view.

==> dependency-tree.tex <==
Here is a small dependency tree showing how the main result of this text, Theorem \ref{thm:main}, is proven. From bottom to top, the tree displays a rough outline of which statement is used to prove what. Only a small part of all Theorems, Lemmas and Propositions is displayed.

\vspace{4cm}

\Tree% 
[.{Theorem \ref{thm:main}} 
  {Proposition \ref{p:convergence}} 
  [.{Theorem \ref{thm:main2}} 
    [.{Theorem \ref{thm:main3}}
      [.{Theorem \ref{thm:spectral}}
        {Theorem \ref{thm:spectral2}\\(proven in section \ref{sect:Proof-spectral-2})}
      ]
      [.{Theorem \ref{thm:main4}\\(proven in section \ref{sect:Proof-main4})}
        {Theorem \ref{t:group}\\(proven in section \ref{subsect:Proof-of-spectral2-and-group})}
      ]
    ]
  ]
  !\qsetw{3cm} {Formula \eqref{eq:difference-of-the-omega}} 
]

